TurboFFT: A High-Performance Fast Fourier Transform with Fault Tolerance on GPU

The Fast Fourier Transform (FFT), as a core computation in a wide range of scientific applications, is increasingly threatened by reliability issues. In this paper, we introduce TurboFFT, a high-performance FFT implementation equipped with a two-sided checksum scheme that detects and corrects silent data corruptions at computing units efficiently. The proposed two-sided checksum addresses the error propagation issue by encoding a batch of input signals with different linear combinations, which not only allows fast batched error detection but also enables error correction on-the-fly instead of recomputing. We explore two-sided checksum designs at the kernel, thread, and threadblock levels, and provide a baseline FFT implementation competitive to the state-of-the-art, closed-source cuFFT. We demonstrate a kernel fusion strategy to mitigate and overlap the computation/memory overhead introduced by fault tolerance with underlying FFT computation. We present a template-based code generation strategy to reduce development costs and support a wide range of input sizes and data types. Experimental results on an NVIDIA A100 server GPU and a Tesla Turing T4 GPU demonstrate TurboFFT offers a competitive or superior performance compared to the closed-source library cuFFT. TurboFFT only incurs a minimum overhead (7\% to 15\% on average) compared to cuFFT, even under hundreds of error injections per minute for both single and double precision. TurboFFT achieves a 23\% improvement compared to existing fault tolerance FFT schemes.

==> listing/alg-interp.tex <==
\begin{lstlisting}[language=python, caption={The essense of {\ginterp} implementation.}, basicstyle=\ttfamily\footnotesize, 
escapeinside={(*@}{@*)}, morekeywords={fn, reference, volatile, constexpr, parfor},
label={cuszinterp::algo::interp}
]
""" original data value (*@$d$@*), predicted value (*@$p$@*), 
predict. error (*@$e$@*), quant-code (*@$q$@*), error bound (*@$eb$@*), 
radius (*@$r$@*). We refer reader to Tao et al. 
2017 for the detailed pred-quant. algorithm."""
 
fn PerPointPredQuant<sym Direction>(volatile (*@$shm\{data, quant\}$@*), (*@$x$@*), (*@$y$@*), (*@$z$@*), (*@$\alpha$@*)):
    reference (*@$(d, q) \gets (shm.data_{z,y,x}, shm.quant_{z,y,x})$@*)
    (*@$p \gets$@*) Interp<Direction>((*@$x$@*), (*@$y$@*), (*@$z$@*), (*@$\alpha$@*))
    if constexpr COMPRESS: 
        QuantizeComppress((*@$d$@*), (*@$p$@*), (*@$q$@*))
    if constexpr DECOMPRESS: 
        QuantizeDecompress((*@$d$@*), (*@$p$@*), (*@$q$@*))

fn Stage<class Map>(..., Map map):
    if constexpr CORSENING:
        multiply call PerPointPredQuant(...) 
    else:
        one-time call PerPointPredQuant(...)

fn InterpolateIter(volatile (*@$shm\{data, quant\}$@*):
    parfor (*@$\alpha \gets \{4,2,1\}$@*) (predefined parallelism):
        for constexpr (*@$i \gets \{0,1,2\}$@*):
            Stage<(*@$i$@*)>(...)
\end{lstlisting}

==> listing/alg-pred-quant.tex <==
\begin{algorithmic}[1]

	\Statex \textbf{notation:} original data element/value $d$, predicted value $p$, prediction error $e$, quant-code $q$, error bound $eb$,  radius $r$ %(global or captured)

	\Statex
	\Procedure{CompressPredQuant}{\REFERENCE{} $d$, $p$, \REFERENCE{} $q$}
	\State $e \gets d-p$
	\State code $\gets$ \textsc{fabs}($e$)$\,\div\,eb + 1$; code $\gets$ $-$code \INLINEIF{} $e<0$
	\State code $\gets$ \textsc{int}(code$\,\div\,2$) $+\,r$
	\State $q \gets$ code; $d \gets p + (\text{code} - r) \times eb\cdot2$
	\EndProcedure

	\Statex

	\Procedure{DecompressPredQuant}{\REFERENCE{} $d$, $p$, \REFERENCE{} $q$}
	\State $d \gets p + (q - r) \times eb\cdot2$
	\EndProcedure

	\Statex

\end{algorithmic}

==> listing/cr-same-eb-NO-bitcomp.tex <==
\newcommand{\TabDataName}[1]{\rotatebox{90}{\bfseries\scriptsize\scalebox{0.8}{#1}}}
\setlength{\tabcolsep}{4pt}
\scriptsize
\begin{tabular}{|l@{}c|r|r|r|r|r|r|}
  % \hline
  % \multirow{2}{*}{\textbf{Dataset}} &
  % \multirow{2}{*}{\textbf{epsilon}} &
  % \multirow{2}{*}{\textbf{cuSZ}}    &
  % \multirow{2}{*}{\textbf{cuSZp}}   &
  % \multirow{2}{*}{\textbf{cuSZx}}   &
  % \multirow{2}{*}{\textbf{FZ-GPU}}  &
  % \multirow{2}{*}{\textbf{cuSZ-I}}  &
  % \textbf{Improve}                                                                                                                                     \\
  %                                   &       &                     &                     &               &               &                     &
  % \textbf{(\%)}                                                                                                                                        \\

  \multicolumn{1}{l}{\rotatebox{90}{\textbf{Dataset}}} &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{epsilon}}} &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZ}}}    &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZp}}}   &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZx}}}   &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{FZ-GPU}}}  &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZ-I}}}  &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{Improve \%}}}
  \\
  % \hline
  \hline
  \multirow{3}{*}{\TabDataName{RTM}}                   & 1E--2 & 28.7                & \SecondbestCr{41.6} & \NoBcBestCr{53.7} & 32.0              & 28.8                & --46.4 \\ \cline{3-8}
                                                       & 1E--3 & 24.7                & 19.8                & \NoBcBestCr{30.7} & 20.9              & \SecondbestCr{27.4} & --10.7 \\ \cline{3-8}
                                                       & 1E--4 & \SecondbestCr{17.7} & 10.7                & 17.4              & 12.1              & \NoBcBestCr{21.5}   & 21.5   \\ \hline
  \multirow{3}{*}{\TabDataName{Miranda}}               & 1E--2 & 27.1                & 16.8                & 7.9               & \NoBcBestCr{30.6} & \SecondbestCr{28.5} & --6.9  \\ \cline{3-8}
                                                       & 1E--3 & \SecondbestCr{22.9} & 9.6                 & 5.1               & 19.2              & \NoBcBestCr{26.3}   & 14.8   \\ \cline{3-8}
                                                       & 1E--4 & \SecondbestCr{15.3} & 6.0                 & 3.6               & 11.8              & \NoBcBestCr{19.5}   & 27.5   \\ \hline
  \multirow{3}{*}{\TabDataName{S3D}}                   & 1E--2 & \SecondbestCr{28.0} & 7.2                 & 19.5              & 15.5              & \NoBcBestCr{29.5}   & 5.4    \\ \cline{3-8}
                                                       & 1E--3 & \SecondbestCr{23.3} & 4.5                 & 9.3               & 11.8              & \NoBcBestCr{28.8}   & 23.6   \\ \cline{3-8}
                                                       & 1E--4 & \SecondbestCr{17.3} & 3.1                 & 5.0               & 9.0               & \NoBcBestCr{26.0}   & 50.3   \\ \hline
  \multirow{3}{*}{\TabDataName{NYX}}                   & 1E--2 & \NoBcBestCr{30.2}   & 20.3                & N/A               & 25.3              & \SecondbestCr{29.6} & --2.0  \\ \cline{3-8}
                                                       & 1E--3 & \SecondbestCr{23.9} & 9.6                 & N/A               & 14.4              & \NoBcBestCr{28.0}   & 17.2   \\ \cline{3-8}
                                                       & 1E--4 & \SecondbestCr{15.3} & 5.7                 & N/A               & 8.4               & \NoBcBestCr{18.7}   & 22.2   \\ \hline
  \multirow{3}{*}{\TabDataName{JHTDB}}                 & 1E--2 & \SecondbestCr{26.6} & 10.3                & 3.0               & 12.1              & \NoBcBestCr{29.3}   & 10.2   \\ \cline{3-8}
                                                       & 1E--3 & \SecondbestCr{17.7} & 5.4                 & 2.5               & 9.9               & \NoBcBestCr{25.2}   & 42.4   \\ \cline{3-8}
                                                       & 1E--4 & \SecondbestCr{10.7} & 3.5                 & 1.8               & 6.4               & \NoBcBestCr{13.3}   & 24.3   \\ \hline
  \multirow{3}{*}{\TabDataName{Qmcpack}}               & 1E--2 & \SecondbestCr{28.6} & 22.2                & 3.3               & 19.0              & \NoBcBestCr{29.3}   & 2.4    \\ \cline{3-8}
                                                       & 1E--3 & \SecondbestCr{20.9} & 10.1                & 2.5               & 12.1              & \NoBcBestCr{27.7}   & 32.5   \\ \cline{3-8}
                                                       & 1E--4 & \SecondbestCr{14.8} & 5.6                 & 1.9               & 8.3               & \NoBcBestCr{22.6}   & 52.7   \\ \hline
\end{tabular}

==> listing/cr-same-eb-bitcomp.tex <==

\begin{tabular}{|l|c|r|r|r|r|r|r|}
  \hline
  \multirow{2}{*}{\textbf{Dataset}} &
  \multirow{2}{*}{\textbf{epsilon}} &
  \multirow{2}{*}{\textbf{cuSZ}}    &
  \multirow{2}{*}{\textbf{cuSZp}}   &
  \multirow{2}{*}{\textbf{cuSZx}}   &
  \multirow{2}{*}{\textbf{FZ-GPU}}  &
  \multirow{2}{*}{\textbf{cuSZ-I}}  &
  \textbf{Improve}                                                                                                              \\
                                    &       &                     &                      &      &      &                &
  \textbf{(\%)}                                                                                                                 \\
  \hline
  \hline
  \multirow{3}{*}{\textbf{RTM}}     & 1E--2 & 84.1                & \SecondbestCr{100.5} & 70.4 & 69.7 & \BestCr{234.0} & 132.8 \\ \cline{2-8}
                                    & 1E--3 & \SecondbestCr{50.2} & 31.1                 & 38.8 & 35.5 & \BestCr{96.2}  & 91.6  \\ \cline{2-8}
                                    & 1E--4 & \SecondbestCr{26.6} & 14.0                 & 21.4 & 18.4 & \BestCr{45.4}  & 70.7  \\ \hline
  \multirow{3}{*}{\textbf{MIRANDA}} & 1E--2 & \SecondbestCr{67.4} & 18.7                 & 8.1  & 43.9 & \BestCr{174.0} & 158.2 \\ \cline{2-8}
                                    & 1E--3 & \SecondbestCr{38.5} & 10.7                 & 5.2  & 27.1 & \BestCr{77.2}  & 100.5 \\ \cline{2-8}
                                    & 1E--4 & \SecondbestCr{19.8} & 6.7                  & 3.7  & 15.4 & \BestCr{34.3}  & 73.2  \\ \hline
  \multirow{3}{*}{\textbf{S3D}}     & 1E--2 & \SecondbestCr{42.5} & 18.9                 & 19.9 & 25.6 & \BestCr{245.0} & 476.5 \\ \cline{2-8}
                                    & 1E--3 & \SecondbestCr{28.3} & 8.8                  & 9.5  & 16.1 & \BestCr{137.0} & 384.1 \\ \cline{2-8}
                                    & 1E--4 & \SecondbestCr{19.0} & 5.0                  & 5.1  & 11.6 & \BestCr{58.2}  & 206.3 \\ \hline
  \multirow{3}{*}{\textbf{NYX}}     & 1E--2 & 71.6                & \SecondbestCr{95.9}  & N/A  & 84.5 & \BestCr{256.0} & 166.9 \\ \cline{2-8}
                                    & 1E--3 & \SecondbestCr{34.4} & 19.0                 & N/A  & 26.2 & \BestCr{66.1}  & 92.2  \\ \cline{2-8}
                                    & 1E--4 & \SecondbestCr{17.9} & 7.5                  & N/A  & 12.3 & \BestCr{25.1}  & 40.2  \\ \hline
  \multirow{3}{*}{\textbf{JHTDB}}   & 1E--2 & \SecondbestCr{27.8} & 19.9                 & 3.1  & 18.0 & \BestCr{132.0} & 374.8 \\ \cline{2-8}
                                    & 1E--3 & \SecondbestCr{17.7} & 6.0                  & 2.5  & 11.5 & \BestCr{34.8}  & 96.6  \\ \cline{2-8}
                                    & 1E--4 & \SecondbestCr{10.7} & 3.6                  & 1.8  & 7.8  & \BestCr{13.3}  & 24.3  \\ \hline
  \multirow{3}{*}{\textbf{QMCPACK}} & 1E--2 & \SecondbestCr{46.0} & 38.7                 & 3.3  & 30.3 & \BestCr{168.0} & 265.2 \\ \cline{2-8}
                                    & 1E--3 & \SecondbestCr{23.7} & 11.5                 & 2.5  & 14.7 & \BestCr{78.7}  & 232.1 \\ \cline{2-8}
                                    & 1E--4 & \SecondbestCr{15.3} & 5.8                  & 1.9  & 10.2 & \BestCr{34.6}  & 126.1 \\ \hline
\end{tabular}

==> listing/cr-same-eb-combined.tex <==
\begin{tabular}{ >{\color{black}}l@{} >{\color{black}}c| *{2}{c |rrrrr| >{\color{black}}r|} }
  \multicolumn{1}{l}{\rotatebox{90}{\textbf{Dataset}}} &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{epsilon}}} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{\cusz}}}    &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZp}}}   &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZx}}}   &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{FZ-GPU}}}  &
  \multicolumn{1}{r}{\rotatebox{90}{\color{black}\textbf{\thiswork}}}  &
  \multicolumn{1}{r}{\rotatebox{90}{\color{black}\textbf{Improve \%}}} &
  \multicolumn{1}{r}{} &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{\cusz}}}    &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZp}}}   &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{cuSZx}}}   &
  \multicolumn{1}{r}{\rotatebox{90}{\textbf{FZ-GPU}}}  &
  \multicolumn{1}{r}{\rotatebox{90}{\color{black}\textbf{\thiswork}}}  &
  \multicolumn{1}{r}{\rotatebox{90}{\color{black}\textbf{Improve \%}}}
  \\
  \cline{1-2}\cline{4-9}\cline{11-16}
  \multirow{3}{*}{\TabDataName{JHTDB}}                 & 1e--2 && \SecondbestCr{26.6} & 10.3                & 3.0               & 12.1              & \NoBcBestCr{29.3}   & 10.2   &  & \SecondbestCr{27.8} & 19.9                 & 3.1  & 18.0 & \BestCr{132.0} & 374.8 \\
                                                       & 1e--3 && \SecondbestCr{17.7} & 5.4                 & 2.5               & 9.9               & \NoBcBestCr{25.2}   & 42.4   &  & \SecondbestCr{17.7} & 6.0                  & 2.5  & 11.5 & \BestCr{34.8}  & 96.6  \\
                                                       & 1e--4 && \SecondbestCr{10.7} & 3.5                 & 1.8               & 6.4               & \NoBcBestCr{13.3}   & 24.3   &  & \SecondbestCr{10.7} & 3.6                  & 1.8  & 7.8  & \BestCr{13.3}  & 24.3  \\

                                                       
   \cline{1-2}\cline{4-9}\cline{11-16}
  \multirow{3}{*}{\TabDataName{Miranda}}               & 1e--2 && 27.1                & 16.8                & 7.9               & \NoBcBestCr{30.6} & \SecondbestCr{28.5} & --6.9  &  & \SecondbestCr{67.4} & 18.7                 & 8.1  & 43.9 & \BestCr{174.0} & 158.2 \\
                                                       & 1e--3 && \SecondbestCr{22.9} & 9.6                 & 5.1               & 19.2              & \NoBcBestCr{26.3}   & 14.8   &  & \SecondbestCr{38.5} & 10.7                 & 5.2  & 27.1 & \BestCr{77.2}  & 100.5 \\
                                                       & 1e--4 && \SecondbestCr{15.3} & 6.0                 & 3.6               & 11.8              & \NoBcBestCr{19.5}   & 27.5   &  & \SecondbestCr{19.8} & 6.7                  & 3.7  & 15.4 & \BestCr{34.3}  & 73.2  \\
  \cline{1-2}\cline{4-9}\cline{11-16}
  \multirow{3}{*}{\TabDataName{NYX}}                   & 1e--2 && \NoBcBestCr{30.2}   & 20.3                & N/A               & 25.3              & \SecondbestCr{29.6} & --2.0  &  & 71.6                & \SecondbestCr{95.9}  & N/A  & 84.5 & \BestCr{256.0} & 166.9 \\
                                                       & 1e--3 && \SecondbestCr{23.9} & 9.6                 & N/A               & 14.4              & \NoBcBestCr{28.0}   & 17.2   &  & \SecondbestCr{34.4} & 19.0                 & N/A  & 26.2 & \BestCr{66.1}  & 92.2  \\
                                                       & 1e--4 && \SecondbestCr{15.3} & 5.7                 & N/A               & 8.4               & \NoBcBestCr{18.7}   & 22.2   &  & \SecondbestCr{17.9} & 7.5                  & N/A  & 12.3 & \BestCr{25.1}  & 40.2  \\
 
  \cline{1-2}\cline{4-9}\cline{11-16}
  \multirow{3}{*}{\TabDataName{Qmcpack}}               & 1e--2 && \SecondbestCr{28.6} & 22.2                & 3.3               & 19.0              & \NoBcBestCr{29.3}   & 2.4    &  & \SecondbestCr{46.0} & 38.7                 & 3.3  & 30.3 & \BestCr{168.0} & 265.2 \\
                                                       & 1e--3 && \SecondbestCr{20.9} & 10.1                & 2.5               & 12.1              & \NoBcBestCr{27.7}   & 32.5   &  & \SecondbestCr{23.7} & 11.5                 & 2.5  & 14.7 & \BestCr{78.7}  & 232.1 \\
                                                       & 1e--4 && \SecondbestCr{14.8} & 5.6                 & 1.9               & 8.3               & \NoBcBestCr{22.6}   & 52.7   &  & \SecondbestCr{15.3} & 5.8                  & 1.9  & 10.2 & \BestCr{34.6}  & 126.1 \\
\cline{1-2}\cline{4-9}\cline{11-16}
  \multirow{3}{*}{\TabDataName{RTM}}                   & 1e--2 && 28.7                & \SecondbestCr{41.6} & \NoBcBestCr{53.7} & 32.0              & 28.8                & --46.4 &  & 84.1                & \SecondbestCr{100.5} & 70.4 & 69.7 & \BestCr{234.0} & 132.8 \\
                                                       & 1e--3 && 24.7                & 19.8                & \NoBcBestCr{30.7} & 20.9              & \SecondbestCr{27.4} & --10.7 &  & \SecondbestCr{50.2} & 31.1                 & 38.8 & 35.5 & \BestCr{96.2}  & 91.6  \\
                                                       & 1e--4 && \SecondbestCr{17.7} & 10.7                & 17.4              & 12.1              & \NoBcBestCr{21.5}   & 21.5   &  & \SecondbestCr{26.6} & 14.0                 & 21.4 & 18.4 & \BestCr{45.4}  & 70.7  \\
  \cline{1-2}\cline{4-9}\cline{11-16}
  
  \multirow{3}{*}{\TabDataName{S3D}}                   & 1e--2 && \SecondbestCr{28.0} & 7.2                 & 19.5              & 15.5              & \NoBcBestCr{29.5}   & 5.4    &  & \SecondbestCr{42.5} & 18.9                 & 19.9 & 25.6 & \BestCr{245.0} & 476.5 \\
                                                       & 1e--3 && \SecondbestCr{23.3} & 4.5                 & 9.3               & 11.8              & \NoBcBestCr{28.8}   & 23.6   &  & \SecondbestCr{28.3} & 8.8                  & 9.5  & 16.1 & \BestCr{137.0} & 384.1 \\
                                                       & 1e--4 && \SecondbestCr{17.3} & 3.1                 & 5.0               & 9.0               & \NoBcBestCr{26.0}   & 50.3   &  & \SecondbestCr{19.0} & 5.0                  & 5.1  & 11.6 & \BestCr{58.2}  & 206.3 \\
  
  \cline{1-2}\cline{4-9}\cline{11-16}
  
\multicolumn{3}{c|}{} & \multicolumn{6}{c|}{\color{black}\bfseries without Bitcomp} & \multicolumn{1}{c|}{} & \multicolumn{6}{c|}{\color{black}\bfseries {with Bitcomp} } \\
\multicolumn{2}{c}{col. no.} & \multicolumn{1}{c}{} &
1 & 2 & 3 & 4       & \multicolumn{1}{r}{5} & \multicolumn{1}{r}{6} & 
\multicolumn{1}{c}{} & 
i & ii & iii & iv   & \multicolumn{1}{r}{v} & \multicolumn{1}{r}{vi} \\
\end{tabular}

==> listing/cuszi-overview.tex <==
\newcommand{\TableNop}{\multicolumn{1}{c}{}}
\begin{tabular}{ l c |p{11em}| c cc|p{5em}|c|p{9.19em}|}
	\TableNop
	                                              & \TableNop
	                                              &
	\multicolumn{1}{p{11em}}{prediction \& error quantization (with outlier compaction)}
	                                              & \TableNop                          &
	\multicolumn{1}{c}{statistics}                & \TableNop
	                                              &
	\multicolumn{3}{c}{multi-stage lossless encoding}                                                                                                                                                          \\
	\cline{3-3}\cline{5-5}\cline{7-9}
	\TableNop                                     & \TableNop                          & \TableNop                      & \TableNop     &                  & \TableNop     & \TableNop & \TableNop & \TableNop \\
	\cline{3-3}\cline{5-5}\cline{7-7}
	\textbf{cusz}                                 &                                    &
	Lorenzo prediction, dual-quantization variant 
	& \multicolumn{1}{c|}{$\rightarrow$} & \multicolumn{1}{c|}{histogram} & $\rightarrow$ & Huffman encoding & \TableNop     & \TableNop                         \\
	\cline{3-3}\cline{5-5}\cline{7-7}
	\TableNop                                     & \TableNop                          & \TableNop                      & \TableNop     &                  & \TableNop     & \TableNop & \TableNop & \TableNop \\
	\cline{3-3}\cline{5-5}\cline{7-7}\cline{9-9}
	\textbf{cusz-i}                               &                                    &
	linear, qudratic, and cubic spline-interpolation
	                                              & \multicolumn{1}{c|}{$\rightarrow$}                 & \multicolumn{1}{c|}{histogram} & $\rightarrow$ & Huffman encoding & $\rightarrow$ &
	spatial-redundancy elimination                                                                                                                                                                             \\
	\cline{3-3}\cline{5-5}\cline{7-7}\cline{9-9}
\end{tabular}%

==> listing/datasets.tex <==
\begin{tabular}{|rrll|}
\hline  \multicolumn{4}{|l|}{\textbf{JHTDB}~\cite{jhtdb}: numerical simulation of turbulence.} \\
% \hline  
& 10 files    & dim: $zyx = 512\times512\times512$          & total: 5 GB    \\
% \hline
\hline  \multicolumn{4}{|l|}{\textbf{Miranda}~\cite{miranda}: hydrodynamics simulation.} \\
% \hline  
& 7 files & dim: $zyx=256\times384\times384$          & total: 1 GB   \\
% \hline
\hline  
\multicolumn{4}{|l|}{\textbf{NYX}~\cite{nyx}: cosmological hydrodynamics simulation.}  \\
% \hline  
& 6 files & dim: $zyx=512\times512\times512$          & total: 3.1 GB \\
% \hline
\hline  
\multicolumn{4}{|l|}{\textbf{QMCPack}~\cite{qmcpack}: Monte Carlo quantum simlation.}  \\
% \hline  
& 1 files & dim: $zyx=288\times115\times69\times69$ & total: 612 MB \\
% \hline
\hline  
\multicolumn{4}{|l|}{\textbf{RTM}~\cite{rtm}: reverse time migration for seismic imaging.} \\
& 37 files     & dim: $zyx=449\times449\times235$          & total: 6.5 GB \\
% \hline
\hline \multicolumn{4}{|l|}{\textbf{S3D}~\cite{repo-sdrbench}: combustion process simulation.}  \\
% \hline 
& 11 files   & dim: $zyx=500\times500\times500$          & total: 5.1 GB \\
\hline
\end{tabular}

==> listing/tab-testbed.tex <==
\begin{tabular}{ | >{\bfseries}l|c|c|c|}
    \hline
    {GPU}      & \multicolumn{2}{c|}{A100 (40GB)}       & A40 (48 GB)        \\
    \hline
    \hline
    {testbed}  & Theta-GPU    & Anvil        & JLSE         \\
    \hline
    {mem. bw.}  & \multicolumn{2}{c|}{1555 GB/s}    & 695.8  GB/s  \\
    \hline
    {compute}  & \multicolumn{2}{c|}{19.49 TFLOPS} & 37.42 TFLOPS \\
    \hline
    {CUDA/driver}     & 11.4/470.161.03         & 11.6/530.30.02         & 11.8/545.23.06         \\
    \hline
    % {driver}   & 470.161.03   & 530.30.02    & 545.23.06    \\
    % \hline
    % {access}   &
    % \multicolumn{3}{c|}{November, 2023}                     \\
    % \hline
\end{tabular}%

